Measuring Online Emotional Reactions to Events

The rich and dynamic information environment of social media provides researchers, policy makers, and entrepreneurs with opportunities to learn about social phenomena in a timely manner. However, using this data to understand social behavior is difficult due heterogeneity of topics and events discussed in the highly dynamic online information environment. To address these challenges, we present a method for systematically detecting and measuring emotional reactions to offline events using change point detection on the time series of collective affect, and further explaining these reactions using a transformer-based topic model. We demonstrate the utility of the method on a corpus of tweets from a large US metropolitan area between January and August, 2020, covering a period of great social change. We demonstrate that our method is able to disaggregate topics to measure population's emotional and moral reactions. This capability allows for better monitoring of population's reactions during crises using online data.

==> lqbz.tex <==
\begin{table*}[t]
%\addtolength{\tabcolsep}{-2.0pt}
\caption{Top events and the emotional and moral reactions detected by our method,  %Emotion and moral reactions detected in response to offline events, 
in descending order of impact.}
%\\(Impact represented by the number of emotions/moral sentiments changed).}
\centering
\resizebox{1\linewidth}{!}{
\renewcommand{\arraystretch}{1.03}
\begin{tabular}{c|l|l|l|l|l|l}
\Xhline{1pt}
% \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\textbf{Event}}                                                                              & \multicolumn{1}{c|}{\textbf{Date}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Change Point\\ Date Range\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Emotion/Morality\\ that Increased\end{tabular}}}                                                   & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Emotion/Morality\\ that Decreased\end{tabular}}} & \multicolumn{1}{c}{\textbf{Relevant Topics}}                                                                                          \\ \hline
& \textbf{Event} & \textbf{Date} & \textbf{Time Window} & \textbf{Peaking Emotion/MF} & \textbf{Declining Emotion/MF} & \textbf{Relevant Topics} \\ \hline
1                     & \begin{tabular}[c]{@{}l@{}}MLK Jr. Day\end{tabular}                                             & 01-20                              & 01-17 to 01-20                                                                                  & joy, loyalty, fairness                                                                                                                                    &                                                                                                         & \begin{tabular}[c]{@{}l@{}}“mlk, king, martin”,\\ “rights, king, justice”\end{tabular}                                                \\ \hline
2                     & \begin{tabular}[c]{@{}l@{}}Trump’s impeachment\\ trial\end{tabular}                                              & 01-20                              & 01-20 to 01-21                                                                                  & betrayal, subversion                                                                                                                                      &                                                                                                         & \begin{tabular}[c]{@{}l@{}}“senate, vote, will”,\\ “treason, traitors, moscow”\end{tabular}                                           \\ \hline
3                    & Earthquake                                                                                                       & 01-20                              & 01-20                                                                                           & fear                                                                                                                                                      & \textbf{}                                                                                               & “earthquake, usgs, km”                                                                                                                \\ \hline
4                     & Kobe Bryant’s death                                                                                              & 01-26                              & 01-26                                                                                           & \begin{tabular}[c]{@{}l@{}}anger, pessimism, sadness,\\ care, harm, purity\end{tabular}                                                                   & joy                                                                                                     & \begin{tabular}[c]{@{}l@{}}“kobe, rest, peace”, \\ “prayers, praying, family”\end{tabular}                                            \\ \hline
5                     & \begin{tabular}[c]{@{}l@{}}Trump’s State of the\\ Union address\end{tabular}                                     & 02-03                              & 02-03                                                                                           & anger, disgust, authority                                                                                                                                 &                                                                                                         & \begin{tabular}[c]{@{}l@{}}“pelosi, nancy, speech”,\\ “pelosi, trump, tear”\end{tabular}                                              \\ \hline
6                     & Valentine’s Day                                                                                                  & 02-14                              & 02-14                                                                                           & love                                                                                                                                                      & anger, disgust                                                                                          & “valentine, valentines, happy”                                                                                                        \\ \hline
7                     & \begin{tabular}[c]{@{}l@{}}CA Pres. primary\end{tabular}                                       & 03-03                              & 03-02 to 03-03                                                                                  & fairness, subversion                                                                                                                                      &                                                                                                         & \begin{tabular}[c]{@{}l@{}}“vote, california”,“biden”\end{tabular}                                              \\ \hline
8                     & COVID-19 pandemic                                                                                                & 03-10                              & 03-09 to 03-11                                                                                  & \begin{tabular}[c]{@{}l@{}}anger, disgust, fear,\\ sadness, care, harm,\\ authority\end{tabular}                                                          & \begin{tabular}[c]{@{}l@{}}anticipation, joy,\\ love, optimism\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}“coronavirus, corona, virus”,\\ “pandemic, virus, administration”,\\ “safe, stay, everyone”\end{tabular} \\ \hline
9                     & \begin{tabular}[c]{@{}l@{}}DOJ Drops Flynn Case\end{tabular}                       & 05-07                              & 05-07                                                                                           & cheating                                                                                                                                                  &                                                                                                         & “flynn, cheated, cheating”                                                                                                            \\ \hline
10                     & \begin{tabular}[c]{@{}l@{}}BLM protests\end{tabular}                                            & 05-26                              & 05-25 to 05-30                                                                                  & \begin{tabular}[c]{@{}l@{}}anger, disgust, fear, care,\\ harm, fairness, cheating,\\ loyalty, betrayal, authority,\\ subversion, degradation\end{tabular} & \begin{tabular}[c]{@{}l@{}}anticipation, joy,\\ love, optimism\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}“racist, racism, white”,\\ “murder, george, floyd”, \\ “black, injustices, oppresion”\end{tabular}         \\ \hline








%10                    & \begin{tabular}[c]{@{}l@{}}Biden criticizes Trump\\ on Russian bounties\end{tabular} & 06-27                              & 06-27                                                                                           & betrayal                                                                                                                                                  & \textbf{}                                                                                               & \begin{tabular}[c]{@{}l@{}}“trump, traitor, must”,\\ “biden, president, treason”\end{tabular}                                         \\ \hline
%11                    & \begin{tabular}[c]{@{}l@{}}Trump: ”He got caught,\\ OBAMAGATE!”\end{tabular}                             & 05-11                              & 05-11                                                                                           & subversion                                                                                                                                                & \textbf{}                                                                                               & “obama, trump, president”                                                                                                             \\ \hline
11                    & \begin{tabular}[c]{@{}l@{}}Dodgers beat Giants\end{tabular}                                              & 07-23                              & 07-23                                                                                           & joy                                                                                                                                                       & \textbf{}                                                                                               & “dodgers, mlb, giants”                                                                                                                \\ \hline

%14                    & Earthquake                                                                                                       & 04-03                              & 04-03                                                                                           & fear                                                                                                                                                      & \textbf{}                                                                                               & “usgs, reports, quake”   \\                                                                                                             
\Xhline{1pt}
\end{tabular}}
%\addtolength{\tabcolsep}{2.0pt}

\label{tab_reactions}
\end{table*}
